5G Advanced: Wireless Channel Virtualization and Resource Mapping for Real Time Spectrum Sharing

The coexistence between active wireless communications and passive RF spectrum use becomes an increasingly important requirement for coordinated spectrum access supporting critical services. The ongoing research and technological progress are focused on effective spectrum utilization including large-scale MIMO and energy efficient and low-power communications, innovative spectrum use and management, and resilient spectrum sharing, just to name a few. This paper introduces a new tool for real time spectrum sharing among emerging cellular networks and passive RF sensing systems used for remote sensing and radio astronomy, among others. Specifically we propose leveraging wireless channel virtualization and propose a virtual-to-physical resource mapping framework, mapping types, and control signaling that extends the current 5G New Radio (NR) specifications. Our technology introduces minimal changes to the protocol and is meant to be transparent to the end user application. We validate the proposed technology by extending a 3GPP compliant 5G NR downlink simulator and identify further research directions where work is needed on designing effective ways to explicitly signal the need for spectrum or spectrum use predictions.

==> include/Figures_mapping.tex <==


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/Mapping_types/Direct Mapping.pdf}
    \caption{Direct Mapping }
    \label{fig:direct}
    %\vspace{-3mm}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/Mapping_types/freq shiffting mapping .pdf}
    \caption{Mapping by shift to another BWP }
    \label{fig:BWP shift}
    %\vspace{-3mm}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/Mapping_types/Time shift mapping.pdf}
    \caption{Mapping by shift to other time slots}
    \label{fig:time shift}
    %\vspace{-3mm}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/Mapping_types/Mapping type 4.pdf}
    \caption{Mapping by shift to other time slots with change the RBs order}
    \label{fig:time_shift 2}
    %\vspace{-3mm}
\end{figure}


==> include/Frame_RBG.tex <==
\subsection{5G NR carrier structure}
Similar to the LTE, the smallest frequency resource in NR is the Resource Element (RE) which is occupied 1 subcarrier in frequency domain and 1 OFDM symbol, but the smallest frequency resources unit using in the resources assignment is the resources Block (RB). NR RB contains 12 consecutive RE irrespective of the numerology. The bandwidth occupied by the RB depends on the SCS being used as shown in table 2. As the SCS increases, the bandwidth occupied increases. Another important term in the frequency resources is the resource grid which is characterized by one subframe in the time domain and full carrier bandwidth in the frequency domain. Foe each numerology and carrier we have only one resource grid . Number of RBs in the resource grid depends on the numerology used. A single NR carrier is limited to 3300 active subcarriers which yields to maximum number of RB per resources grid being 275 RBs. Fig \ref{fig:grid} shows the full structure of the NR carrier.
To enable more flexibility in the resources assignment and to accommodate with the UE's capability, a new concept of subdivided the carrier bandwidth to different bandwidth parts (BWP). Each BWP is associated with its own numerology (SCS and CP). The BWP contains a set of contiguous common RB (CRBs) within the full carrier bandwidth. A UE can be configured with up to four downlink BWPs and up to four uplink BWPs for each serving cell and it is only assumed to receive/transmit within active DL/UL BWP using the associated numerology. Only one BWP in the downlink and one in the uplink are active at a given time on an active serving cell. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/NR carrier.png}
    \caption{NR carrier structure}
    \label{fig:grid}
    %\vspace{-3mm}
\end{figure}
\subsection{5G NR Frame structure}
 In NR the time frame length is the same as LTE 10 ms, and it contains 10 subframes each of length 1 ms. Subframe was used as the minimum time scheduling unit in LTE and it contains 14 OFDM symbols where in NR due to the introducing of the new SCS's the OFDM symbol is used as the minimum time scheduling unit. The only SCS used in LTE is 15 kHz where in NR we have 15, 30, 60, 120 and 240 kHz and this made the structure of the subframe differ from LTE. The subframe length still 1 ms and it is the same for all SCS, but the number of slots per subframe and the duration of the OFDM symbol depend on the SCS and numerology.  As we are going higher in the numerology/SCS the number of slots/subframe is duplicated and the symbol duration decreases to the half. Number of OFDM symbols per slot is fixed for all SCS, it is 14 OFDM symbols for normal cyclic prefix (CP) and 12 in the case of extended CP. The NR frame structure and how it depends on the SCS is shown in figure \ref{fig:frame}. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/frame_structure_new.eps}
    \caption{NR Frame Structure (\hl{fonts size of text/numbers in figure needs to be much larger})}
    \label{fig:frame}
    %\vspace{-2mm}
\end{figure}


==> include/RAF.tex <==
Physical downlink shared channel (PDSCH) and Physical uplink shared channel (PUSCH) are used to carry user data for downlink/uplink data transmission from the gNB toward the UEs and visa versa. PDSCH is transmitted in the dL direction from the gNB to the UEs and it contains DL user data, UE specific higher layer information, system information, and paging. In the other hand, PUSCH is transmitted in the UL direction from the UEs to the gNB and it carries both signalling and user data in addition to uplink control information (UCI).These data channels are mapped to a set of time\_frequency resources which are  assigned by the MAC scheduler for transmission. MAC scheduler can be programmed to support one scheduling algorithm such as Round Robin(RR), Proportional Fairness(PF), and Best Channel State Information(Best\_CSI). In addition to the scheduling algorithm, the scheduler is restricted by the allocation types used to allocate resources which are discussed more in the next subsections.

The gNB informs the UEs about the set of frequency\_time resources allocated by encoded the scheduling information in the downlink control channel (DCI) which is carried by the Physical Downlink Control Channel (PDCCH).Once the UE detect a valid PDCCH it extract the DCI and decode the scheduling information to check where it expects to receive data in the case of DL transmission or where it can send data in case of UL transmission. The DCI carries downlink scheduling assignments, uplink scheduling grants and other control information for one UE or a group of UEs. The scheduling information inside the DCI is used to inform the UE which RBs in frequency domain and where in the time slot the UE should look for receiving the PDSCH or to use to send the PUSCH. The DCI data is attached with 24 bits cyclic redundancy check (CRC) which is scrambled with the corresponding identifier  referred to as a radio network temporary identifier (RNTI). Using the RNTI mask, the UE can detect the DCI for its unicast data and distinguish sets of DCI with different purposes that have the same payload size. DCI has different formats depends on the purpose it is used for, these formats and it is specific usage is summarized in table\ref{tab:DCI}. A specific filed in the DCI  0\_0/0\_1/1\_0/1\_1 formats called Frequency domain resource assignment carries the frequency resources scheduling information, and the number of bits for this field is determine by the allocation type used. The scheduler allocates frequency resources to the UEs in three different schemes in the UL direction and two schemes in the DL direction. These different schemes are described in details in the following subsections.
\begin{table}
\centering
\caption{ 5G NR DCI Formats}
\label{tab:DCI}
\begin{tabular}{|p{2.3cm}|p{5.8cm}|}
\hline
\textbf{DCI format}&\textbf{Usage}\\\hline
DCI 0\_0/0\_1 & Scheduling of PUSCH in one cell\\ \hline
DCI 1\_0/1\_1 & Scheduling of PDSCH in one cell \\ \hline
DCI 2\_0&Notifying a group of UEs of the slot format \\ \hline
DCI 2\_1&Notifying a group of UEs of the PRB(s) and OFDM symbol(s) where UE may assume no transmission is intended for the UE \\ \hline

DCI 2\_2&Transmission of TPC commands for PUCCH and PUSCH.\\ \hline

DCI 2\_3&Transmission of a group of TPC commands for SRS transmissions by one or more UEs.\\
\hline
\end{tabular}
\end{table}
\subsection{Frequency Domain Resources Allocation (FDRA) Types}
In 5G NR three uplink resource allocation schemes type 0, type 1 and type 2 and two downlink resource allocation schemes are supported. When the resources allocation is received via DCI Formats 0\_0/1\_0 type 1 is always used  except when the RRC parameter useInterlacePUCCH-PUSCH is set to 'enabled' in which case uplink resource allocation type 2 is used. The MSB bit in the frequency domain resources assignment filed in the DCI format 0\_1/1\_1 is used to indicate which type to use, 0 means type 0 where 1 means type 1. Uplink Resource allocation type 2 should be used for DCI format 0\_1 if the RRC parameter useInterlacePUCCH-PUSCH is set to 'enabled'.

\subsubsection{Downlink / Uplink frequency resources allocation type 0}
Resource allocation type 0 is a bitmap scheme such that the resource allocation information includes a bitmap indicate the resources block groups(RBG's) which allocated to the UE to transmit/receive data on. The RBG is a set of virtual consecutive RB's and the number of RB's in the RBG is determined by two parameters, a higher layer parameter rbg-Size configured by PDSCH/PUSCH-Config and the size of the BWP as shown in table 3. The number of RBGs $N_{RBG}$ in a BWP  of size $N_{BWP}^{size}$ is determined based on the number of RB's in the RBG and the size of the BWP.\\
Number of bits needed to map the RBGs to the UE is equal to $N_{RBG}$. An RGB is allocated to the UE if its corresponding bit value in the bitmap is 1, and it is not allocated if the bit value is 0  . The RGB bitmap are mapped from MSB to LSB, where MSB is for the $RBG_{0}$  and LSB is for $RBG_{N_{RGB}-1}$. An example of type 0 allocation is shown in Fig \ref{fig:type0}. We can see in the figure how the resources blocks allocated to the UE are distributed through the active BWP which gives more flexability comparing to the other types but with the cost of adding more bits in the resources allocation field within the DCI.  

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/resources_allocation_type0_updated_1.eps}
    \caption{ Example on PDSCH Resources Allocation Type 0, the active BWP size is 31 RB's and it starts at CRB 10,the BWP is divided to 9 RBG each with size 4 RB's expect the first and the last RBG they have 2 and 1 RB's size respectively, the UE is assigned 5 RBG based on the bitmap [101101010]}
    \label{fig:type0}
    %\vspace{-2mm}
\end{figure}
\subsubsection{Downlink / Uplink frequency resources allocation type 1}
In the resources allocation type 1, the UE is assigned contiguous VRBs to use them for downlink/uplink data. The network encode the starting virtual resource block ($RB_{start}$) and the length of the contiguously allocated RBs ($L_{RBs}$) in a resource indication value (RIV) in the  resource allocation field. The UE decodes the RIV value to know where to send/receive data. When the resources scheduling grant is received using DCI format 0\_0/0\_1/1\_0/1\_1, the RIV is calculated  using the BWP size, the $L_{RBs}$ and the start RB. 
Where if the  resources scheduling grant is received using DCI format 0\_2/1\_2, the starting RBG and the length  of virtually contiguously allocated RBGs are used to calculate the RIV. The $N_{RBG}$ depends on the RBG size which is provided by the RRC parameter ResourceAllocationType1-granularity-ForDCIFormat0\_2/1\_2 within PUSCH/PDSCH-Config IE. RBG could be 2,4,8, or 16 RBs. If this field is not configured, RBG should be set to 1. 
Fig \ref{fig:type1} shows two examples on type 1 resources allocation using both DCI formats, we can see how the unit of allocation is different in both cases.

\begin{figure}%
\centering
    \subfloat[\centering Using DCI format 1\_0/1\_1]{{\includegraphics[width=8cm]{figures/resources_allocation_type1_1_update.eps} }}%
    \qquad
    \subfloat[\centering Using DCI format 1\_2 ]{{\includegraphics[width=8cm]{figures/resources_allocation_type1_2.eps} }}%
    \caption{Two examples on PDSCH Resources Allocation Type 1, for both examples the active BWP size is 31 RB's and it starts at CRB 10,for a the UE allocated 15 consecutive VRB and the start RB is VRB 4 within the active BWP, in B the active  BWP is divided to 9 RBG each with size 4 RB's expect the first and the last RBG they have 2 and 1 RB's size respectively and the UE is assigned 5 consecutive RBGs which contain 20 VRBs ans starts at RBG 2 within the active BWP}%
    \label{fig:type1}%
\end{figure}

\subsubsection{Uplink frequency resources allocation type 2}
Resources allocation type 2 is only available for the uplink, it doesn't used for the downlink shared channel. When the RRC parameter useInterlacePUCCH-PUSCH is set to 'enabled' resources allocation type 2 is used. This type is only used for SCS 15 and 30 kHz where 5 or 10 interlaces  RBs (IRBs) are defined  depends on the SCS. An interlace m ∈ {0, 1, ..., M−1} consists of common RBs {m, M+m, 2M+m, 3M+m,...}, with M being the number of interlaces. If the active UL BWP uses 5 kHz SCS, 10 IRBs are defined and 6+Y bits provide the frequency domain resource allocation. The 6 MSBs contains the RIV value which Indicates the starting interlace index and the number of contiguous interlace indices. For the 30 kHz SCS case, 5 IRB's are defined and 5+Y bits are used for the frequency domain resource allocation. The 5 MSB's comprise a bitmap indicating the interlaces that are allocated to the scheduled UE. The Y bits for both SCS are used to indicate  RB set allocation inside the IRB's assigned to the UE. The value of Y is determined by Ceil (log2(N(N+1)/2)), where N the number of RB sets contained in the BWP. Figure \ref{fig:type2} shows an example for this type.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/resources_allocation_type2.eps}
    \caption{ Resources Allocation Type 2}
    \label{fig:type2}
    %\vspace{-2mm}
\end{figure}




%The frequency and time resources allocation have been discussed in sections \ref{sec:FDS} and \ref{sec:TDS} is the responsibility of the scheduler which is ruining in the MAC layer at the gNB. The functions of the scheduler is to decide which UE should transmit or received for each kth slots and allocate the needed virtual frequency resource blocks and OFMD symbols to this UE. The decision is made based on number of factors such as the buffer size of the UE in case of uplink grant, the CSI,fairness, services KPI, and other factors depending on the how the scheduler is designed. As mentioned in section \ref{sec:FDS} the UE is assigned VRBs within the active BWP and these VRBs are mapped to Physical resource blocks(PRB) in the last step of the physical layer at the gNB side as shown in figure \textcolor{red}{figure}. The VRB to PRB mapping is a new concept which was introduced in the 5G NR to add more flexibility with decreasing the control signal overhead and to handle the variation in the channel quality specially for high mobility devices. Two type of mapping are used for VRB-PRB mapping, non-interleaved and interleaved mapping and the . With the non-interleaved mapping the VRBs in the BWP  are directly mapped to the same PRB in the BWP with no interleaving procedure. This method is used with type 0 frequency resources  allocation where the allocated RB's are already distributed across the BWP and the frequency diversity is achieved. Also, this mapping scheme could be used with type 1 frequency resources allocation when channel-dependent scheduler is used where the scheduler assign contiguous VRBs with the best channel condition to the selected devices, so if the allocated VRBs distributed across the BWP in the mapping procedure it will result in using RBs with worse channel condition that the allocated one. Therefore, it is better to keep the location of the allocated VRBs as given from the scheduler.  
 %The other mapping method is the interleaving with using an interleaver that takes the contiguous allocated VRBs and distributed it through the whole BWP to enable frequency diversity when the channel condition is not used in the scheduler decision or it is hard to follow the rabid variation of the channel condition during the time due to the high mobility of the devices. In addition to that this scheme could be used  when the  allocation spans the whole BWP with channel quality variation to help in quality averaging across the transport block. The interleaving mapping works on map the VRB to PRB in different location in the BWP and it mapped every 2 or 4 RBs together depends on higher layer signaling. More details about both mapping schemes can be gained from the example shown in figure \textcolor{red}{fig} which illustrate how the both schemes work. 
%\hl{Maybe we can just explain the V-t-P mapping technology and skip discussing the sensor needs here but provide practical examples in the next section?}

%\hl{Do we need to talk so much about OFDMA?}
%\textcolor{blue}{context of resource mapping at the PHY layer of 4G or 5G or any OFDMA based system. This we consider virtual resource mapping and the scheduled resources we consider virtual resources For mapping to physical resources, we introduce the diagram how it works flowchart or block diagram of a simplified transmitter}

%Orthogonal frequency division multiple access (OFDMA) is a multiple access variant of orthogonal frequency division multiplexing (OFDM), which divides the available spectrum into a number of multiplexed orthogonal subcarriers, each one being modulated by a low rate data stream.  %Due to the lower rate symbol stream of subcarriers and insertion of guard time interval to each symbol, the OFDMA system have a good ability to deal with channel time dispersion caused by multipath time delay spread.
%OFDMA has been employed by the the xG  mobile wireless network starting with 4G system where it has been used for the downlink (base station to mobile device) with a fixed subcarrier spacing (SCS) of 15 kHz and QPSK, 16QAM or 64QAM modulation scheme on the subcarriers. The 5G New Radio (NR) standard continues to use OFDMA on both the uplink and downlink with a several SCS options (15 kHz, 30 kHz, 60 kHz, 120 kHz, 240 kHz, 480 kHz) and modulation schemes (QPSK, 16QAM, 64QAM or 256QAM). 
%\hl{Is the. next related to guard band, what does it have to do with OFDMA and why is this relevant here?} By using OFDMA, the 4G LTE network was able to achieve a bandwidth utilization of 90 percent based on the number of usable radio blocks. By further improving the filtering and the precoding technology, OFDMA in 5G enhances the system bandwidth utilization to 98 percent based on the number of usable radio blocks. %Given that performance improvement, OFDMA is most likely continue being used on the 6G system. Therefore, we are going to design our mapping algorithm to be compatible with the OFDMA system.  
%While there are other waveform proposals, OFDM will continue to have an impact in wireless communications. 

==> include/RAT.tex <==
Time domain scheduling is dealing with signaling the active UE's with the time resources inside the time frame that should be used to transmit or received data. 
In LTE the UL/DL changes were only possible at subframe level, but in NR the scheduling happens in slot or OFDM symbol level depends on the duplex scheme being used which added more flexibility. In the of Frequency Division Duplex (FDD) the whole slot for a downlink carrier are used for PDSCH, and the whole slot for a uplink carrier is used for PUSCH except the OFDM symbols that defined by DCI format 2\_1 where the UE assume no transmission is intended to the UE in these symbols. In the case of Time Domain Duplex (TDD), there is 3 type of scheduling or configuration in NR, dynamic, static and semi static configuration. The dynamic configuration is done using the PDCCH via the DCI formats where the static and semi static configuration are done using RRC signaling. 

\subsection{Dynamic slot configuration}
In the dynamic scheduling there is no fixed allocation for the UL/DL transmission. The time resources are dynamically scheduling to adapt the traffic load variation and the resources allocation is totally under the control of the scheduler. The scheduler should track the traffic variation, channel state information(CSI), the transmission / retransmission requests from UE's and the buffer size to adapt the scheduling and the allocation of the time resources to DL/UL transmission. The time resources are assigned to the UE's using the control channel PDCCH in the DCI format, DCI format 1\_0,  or 1\_1 for the PDSCH and the  DCI format 0\_0,  or 0\_1 for the PUSCH. The 4 bits time domain resource assignment field value (m) in the DCI data points to row number m+1 r within the lookup tables. Each look up table contains up to 16 row, each row has parameters help the UE to find the time resources that has been assigned to it. \textcolor{red}{Table 3} listed these parameters and their interpretation. The offset parameter (K0 in case of DL and K2 for UL) used to indicates the location of the slot where the reception/transmission of the data happens as the slot where the DCI received is the  reference point. Also, the numerology of the PDCCH and PDSCH/PUSCH  are used to determine the slot. The receiving and transmitting of the payload data can be happened in the same slot where the DCI received, in this case the slot is called self contained slot. The starting symbol and number of symbols inside the slot been used for transmission/receiving are determine by the Start and length Indicator Value (SLIV) or can be directly listed in the table as  start symbol ‘S’ and the allocation length ‘L’. There is a restriction in the validation of the combination of S and L due to the fact that a single time-domain resource allocation must be contained within a slot and there is 14 OFDM symbols (Normal CP) or 12 OFDM symbols (Extended CP) within one slot and the combination should take this into consideration, like we can't start from symbol 7 and have 10 symbols for transmission/receiving. The last parameter in the table is used to know the mapping type. There are two mapping type related to the relative location of the demodulation reference signal (DM-RS) and the slot boundary as well as the size of the data. The first mappying type A used when the first DM-RS symbol is located in the second or third symbol of the slot relative to the slot boundary regardless the  location of the first symbol used for PUSCH/PDSCH, and it is primarily intended for the cases where the data occupies most of the slot. The second mapping type is type B, where the location of the first DM-RS is not given relative to the slot boundary, but it is given relative to the first symbol used for PUSCH/PDSCH where The DM-RS location is the first OFDM symbol allocated to the PUSCH/PDSCH. Mapping type B is used when the data occupied small fraction of the slot and when the transmission can't wit until the start of the slot boundary to support low latency transmission. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/time_allocation.eps}
    \caption{ Example on the dynamic slot configuration and PDSCH resources allocation, the active BWP size is 31 RBs and it starts at CRB 10, the time duration is 2 ms with SCS 30 khz, the UE is allocated VRB in slot 1/subframe 0 and slot 0/subframe 1, each occuipied 6 OFDM symboles and starts at symbole 7 within the slot, the di  }
    \label{fig:type2}
    %\vspace{-2mm}
\end{figure}

\subsection{Static and Semi Static Configuration}
In static and semi static configuration the UE doesn't need to monitor the control channel to know which slot and symbols are assigned for DL or UL transmissions, rather the UE as predefined information about the exact location of the symbols/slots used for UL, DL or fixed where fixed mean that the symbols/slots can be used for DL or UL. This type of scheduling consumes less power than the dynamic one but it is less flexible. It can be use in large cells where there is a lot of users  or where the traffic amount doesn't change too much and it is pretty much fixed. In Static configuration the network informs all the UEs within the cell about the slots/symbols configuration by broadcasting the IE tdd-UL-DL-ConfigurationCommon via system information block (SIB1) or configured to the UE using dedicated RRC signalling. The IE tdd-UL-DL-ConfigurationCommon contains parameters on cell-specific level slots that used to define the  DL/UL pattern over a period of time. The tdd-UL-DL-ConfigurationCommon should contains at least one pattern and it can contains two patterns where 2nd pattern is concatenated onto the 1st pattern and add more flexibility. The pattern defines the periodicity where the DL/UL pattern is repeated, number of slots fully used for DL, number of slots fully used for UL, number of symbols used for DL within the slot that  immediately following the last full DL slot and the number of symbols used for UL within th slot  preceding the first full UL slot. All of the mentioned parameters are defined over the slot configuration period, the remaining unclassified slots and symbols within the configuration period are used as flexible where they can be configured to be used as DL or UL in the semi static configuration.\ 

The semi static configuration is UE-specific level configuration where the network modified the DL/UL pattern based on specific UE need which add more flexibility and allow the network to accommodate with the UE traffic changing. The network informs the specific UE about the updated slot configuration using IE tdd-UL-DL-ConfigurationDedicated which only configures the flexible slots and symbols and can't change the slots and symbols that already allocated for DL/UL via tdd-UL-DL-ConfigurationCommon. The IE tdd-UL-DL-ConfigurationDedicated provides individual slot configuration, it contains parameters help to indicate which slot within the Configuration period needs to be allocated and if the slot is fully dedicated to DL or UL or explicit number of symbols within the slot used for DL and other for UL. Also, the slot can be configured as explicit and number of symbols within it used for DL or UL and the remaining symbols stay flexible. 














































==> include/VRMFold.tex <==

The virtual resources block (VRB) has been introduced in %concept starts with the 
3GPP Release 15 for 5G NR. % where the scheduler at the MAC layer allocates VRBs to the different user equipments (UEs) for data transmission. 
VRBs contain the modulation symbols that are mapped to physical resource blocks (PRBs) within the active bandwidth part (BWP) %used for transmission in the last step 
as part of the physical layer processing at the gNodeB. The VRB-to-PRB mapping was introduced in 5G NR to add more flexibility for radio resources allocation while decreasing the control signaling overhead. It is meant for offering frequency diversity to handle the variations in the channel quality especially for high mobility devices \cite{5gBook}.

The 3GPP specifications support two types of downlink resource allocation in the frequency domain. %  are supported type 0 and type 1.
For both types, the gNodeB assigns VRBs to UEs, but the continuity of the allocated RBs and the number of bits used to inform the UEs about the allocation differ between the two types. Type 0 groups the available RBs in the BWP in virtual resources block groups (VRBGs). % which %and these RBGs 
%are allocated to the UEs.
%The UE  Different 
One or more contiguous or non-contiguous VRBGs within the BWP can be allocated to a UE. For example, %and it does not need to be continuous means the 
VRBGs 1 and 5 may be allocated to a UE. % can be allocated  as an example. 
Resources allocation Type 1, on the other hand, assigns contiguous VRBs to each UE % is assigned  and it can not be assigned noncontagious VRBs
\cite{data}.

The gNodeB informs the UEs about the set of RBs and orthogonal frequency division multiplexing (OFDM) symbols allocated for data transmission by encoding the scheduling information in the downlink control channel (DCI) which is carried by the Physical Downlink Control Channel (PDCCH) \cite{DCI}. Once the UE detects a valid PDCCH it extract the DCI and decodes the scheduling information to find out where to expects the downlink data %in the case of DL transmission 
or where it can send data in the uplink. % case of UL transmission. 
The different types of DCI formats are illustrated in table \ref{tab:DCI} \cite{DCI}. Resource allocation Type 0 employs bit mapping. That is, the number of bits %inside the DCI 
that are needed %to be used 
to inform the UE about the allocated VRBGs is equal to the number of VRBGs within the BWP. For Type 1, the gNodeB encodes the starting virtual resource block ($RB_{start}$) and the length of the contiguously allocated RBs ($L_{RBs}$) as a resource indication value (RIV) in the resource allocation field of the DCI. This requires fewer bits than for Type 0. In conclusion, Type 0 provides more flexibility than Type 1, but it needs more control bits to inform the UEs about the RB allocation.

%Going back the virtual to physical resources mapping,
There are tow types of virtual-to-physical resource mapping supported in the 3GPP specifications, the non-interleaved and interleaved mapping as shown in Figs. \ref{fig:mapping_typs}a and b. For the non-interleaved mapping method, the VRBs in the BWP are directly mapped to the same PRB in the BWP. % with no interleaving procedure. 
The interleaved mapping uses an interleaver that takes the contiguous VRBs and distributes the within the BWP. 

Non-interleaved mapping can be used for both allocation types, type 0 and type 1, where the interleaved mapping is only used with type 1. The reason behinds not using the interleaved mapping with type 0 is that the the allocated RBs are already distributed across the BWP in Type 0 and the frequency diversity is achieved, where in Type 1 as mentioned early the UEs cannot be assigned distributed RBs but with the interleaved mapping the allocated RBs for the UEs can be distributed across the BWP with less overhead control bits. 

Non-interleaved mapping is recommended to use with type 1 allocation scheme when channel-dependent scheduler is used where the scheduler assign contiguous VRBs with the best channel condition to the selected devices, so if the allocated VRBs distributed across the BWP in the mapping procedure it will result in using RBs with worse channel condition than the allocated one. Therefore, it is better to keep the location of the allocated VRBs as given from the scheduler. Interleaved mapping is recommended to use with type 1 when the channel condition is not used in the scheduler decision or it is hard to follow the rabid variation of the channel condition during the time due to the high mobility of the devices.  In addition to that this scheme could be used  when the resources allocation for one UE spans the whole BWP with channel quality variation to help in quality averaging across the transport blocks.

\begin{table}
\centering
\caption{ 5G NR DCI Formats}
\label{tab:DCI}
\begin{tabular}{|p{2cm}|p{6cm}|}
\hline
\textbf{DCI format}&\textbf{Usage}\\\hline
DCI 0\_0/0\_1/0\_2 & Scheduling of PUSCH in one cell \\ \hline
DCI 1\_0/1\_1/1\_2 & Scheduling of PDSCH in one cell \\ \hline
DCI 2\_0&Notifying a group of UEs of the slot format \\ \hline
\rowcolor{LightCyan}
\textbf{DCI 2\_1}&{Notifying a group of UEs of the PRB(s) and OFDM symbol(s) where UE may assume no transmission is intended for the UE} \\ \hline
DCI 2\_2&Transmission of TPC commands for PUCCH and PUSCH.\\ \hline
DCI 2\_3&Transmission of a group of TPC commands for SRS transmissions by one or more UEs.\\
\hline
\end{tabular}
\end{table}

\begin{figure*}
\centering
\vspace{-5mm}
\subfloat[5G NR Non-interleaved resource mapping] 
{\includegraphics[width=3.6in]{figures/Direct_mapping.png}}
\subfloat[5G NR Interleaved resource mapping]
{\includegraphics[width=3.6in]{figures/inter_mapping.png}}\\
\subfloat[Proposed 5G Advanced virtual to physical resource mapping]
{\includegraphics[width=3.6in]{figures/New_mapping.png}}
\caption{Virtual-to-physical resource mapping in 5G NR (a, b) and for 5G Advanced (c).}
\label{fig:mapping_typs}
\end{figure*}












==> include/formula.tex <==
The number of RBGs $N_{RBG}$ in a BWP  of size $N_{BWP}^{size}$ is
\begin{equation*}
   N_{RBG} = \left \lceil{(N_{BWP}^{size} + (N_{BWP}^{start}\mod P))/P}\right\rceil
\end{equation*}
$N_{BWP,i}^{start}$ is the start RB of $BWP_i$. The size of the first and last RBGs are differ from other RBG and are given by the following formulas:
\begin{equation*}
RBG_{0}^{size} = P - N_{BWP}^{start} \mod P
 \end{equation*}  
 If
\begin{equation*}
(N_{BWP}^{start}+ N_{BWP}^{size}) \mod P \geq 0
\end{equation*}  
\begin{equation*}
RBG_{last}^{size} = (N_{BWP}^{start}+ N_{BWP}^{size}) \mod P
 \end{equation*}  
 else,
 \begin{equation*}
   RBG_{last}^{size}=  P
    \end{equation*}   
The size of all other RGBs is P.\\

the RIV is calculated by using the BWP size, the $L_{RBs}$ and the start RB. 
\begin{equation*}
( L_{RBs} - 1 ) \geq \left \lfloor{(N_{BWP}^{size}/2}\right\rfloor 
 \end{equation*}
 \begin{equation*}
RIV = N_{BWP}^{size} * ( L_{RBs} - 1 ) + RB_{start}
\end{equation*}
else
\begin{equation*}
RIV = N_{BWP}^{size} * ( N_{BWP}^{size} - L_{RBs} +1 ) + ( N_{BWP}^{size} - 1 - RB_{start}) 
\end{equation*}

Where if the  resources scheduling grant is received using DCI format 0\_2/1\_2, we used the RBG the RIV is calculated using the $L_{RBGs}$  
If 
\begin{equation*}
( L_{RBGs} - 1 )\geq \left \lfloor{(N_{RBG}/2}\right\rfloor
\end{equation*}
\begin{equation*}
RIV = N_{RBG}^{size}* ( L_{RBGs} - 1 ) + RBG_{start} 
\end{equation*}
else
\begin{equation*}
RIV = N_{RBG} * ( N_{RBG} - L_{RBGs} +1 ) +  ( N_{RBG} - 1 - RBG_{start}) 
\end{equation*}

==> include/table.tex <==
\begin{center}
\begin{table}[ht]
\caption{ 5G NR DCI Formats}
\begin{tabular}{|p{2cm}|p{3cm}|}
\hline
\textbf{DCI format}& \textbf{Usage} \\

\hline

DCI 0\_0 & Fallback DCI format for scheduling of PUSCH 
\\ \hline


DCI 0__1 & Non-fallback DCI format for scheduling of PUSCH

\\ \hline

DCI 1_0 &

Fallback DCI format for scheduling of PDSCH

\\ \hline
DCI 1_1 &

Non-fallback DCI format for scheduling of PDSCH

\\ \hline

DCI 2_0 &

Notifying a group of UEs of the slot format

\\ \hline
DCI 2_1 &

Notifying a group of UEs of the PRB(s) and OFDM symbol(s) where UE may assume no transmission is intended for the UE

\\ \hline

DCI 2_2 &

Transmission of a group of power control commands for PUCCH and PUSCH

\\ \hline

DCI 2_3 &

Transmission of a group of SRS requests and power control commands for SRS transmissions

\\ \hline
\label{tab:DCI}
\end {tabular}
\end{table}
\end{center}

\begin{center}
\begin{table}[ht]
\caption{ Bandwidth occupied by an NR RB}
\begin{tabular}{|p{2cm}|p{3cm}|}
\hline
\textbf{SCS}& \textbf{Bandwidth per RB = 12 x SCS} \\

\hline

15 kHz & 180 kHz
\\ \hline


30 kHz & 360 kHz

\\ \hline

60 kHz & 720 kHz

\\ \hline
120 kHz & 1440 kHz

\\ \hline

240 kHz & 2880 kHz
\\ \hline



\label{tab:RBS}
\end {tabular}
\end{table}
\end{center}


